A Systematic Assessment on Android Third-party Library Detection Tools

Third-party libraries (TPLs) have become a significant part of the Android ecosystem. Developers can employ various TPLs to facilitate their app development. Unfortunately, the popularity of TPLs also brings new security issues. For example, TPLs may carry malicious or vulnerable code, which can infect popular apps to pose threats to mobile users. Furthermore, TPL detection is essential for downstream tasks, such as vulnerabilities and malware detection. Thus, various tools have been developed to identify TPLs. However, no existing work has studied these TPL detection tools in detail, and different tools focus on different applications and techniques with performance differences. A comprehensive understanding of these tools will help us make better use of them. To this end, we conduct a comprehensive empirical study to fill the gap by evaluating and comparing all publicly available TPL detection tools based on six criteria: accuracy of TPL construction, effectiveness, efficiency, accuracy of version identification, resiliency to code obfuscation, and ease of use. Besides, we enhance these open-source tools by fixing their limitations, to improve their detection ability. Finally, we build an extensible framework that integrates all existing available TPL detection tools, providing an online service for the research community. We release the evaluation dataset and enhanced tools. According to our study, we also present the essential findings and discuss promising implications to the community. We believe our work provides a clear picture of existing TPL detection techniques and also gives a roadmap for future research.

==> Approach.tex <==
\section{Approach}
\label{sec:approach}

\begin{figure*}[thpb]
	\centering
	\includegraphics[width=0.85\textwidth]{libhunter}
	\caption{Overview of \mytool}
	\label{fig:libhunter_arch}
\end{figure*}

To address the limitations in the existing TPL detection approaches, we propose and implement a novel system, 
%especially for the module decoupling process, 
which is able to detect newly-emerging TPLs in Android apps and obfuscation-resilient.
We highlight that the module decoupling process in our proposed approach is different from the existing approaches, which makes us achieve a better performance compared with them.
Our proposed system, named \mytool, takes as input an Android app, and automatically identify the TPLs used by the app. Different from existing TPL detection techniques that can only identify libraries in their pre-constructed database, \mytool does not rely on the completeness of the library database which is used to compare with the candidate libraries. Instead, owing to its decoupling strategy and extracted obfuscation-resilient features, it can even start without a database to identify TPLs, create a database and self-augment it iteratively. 

Figure~\ref{fig:libhunter_arch} shows the overview of \mytool, including three key phases:
% that are similar to the existing approaches: %(1) preprocessing, which decompiles the apk file; 
%(1) \textit{Decompiling}, which decompiles the apk file to smali files;
(1) \textit{Module decoupling} splits the TPLs from the host app by constructing the component transition graph (CTG) and package dependence graph (PDG). We first delete the code related to the host app (i.e., primary module) based on the CTG and further identify the code related to each TPL from the no-primary module as library candidates based on PDG;
(2) \textit{Feature extraction}, which generates the control-flow graph (CFG) of each method in the library candidates as the features to represent each candidate;
(3) \textit{Similarity comparison} identifies the concrete library by comparing the features with the libraries in the database (if any) to see whether it exceeds the threshold (i.e, 80\% in our approach). If there is no such a database, we create a new one, and add the first candidate library to the database. Once the database exists, the other candidate libraries should first compare with the ones in databases. If no libraries in the database are similar enough to the candidate (i.e., below threshold), it is considered as a new library and added to the database, which highlights that our library database can self-augment by the identified newly-emerging TPLs.
Next, we introduce the details of some key phases in \mytool.

%(1) \textbf{Candidate library extraction}, which splits the suspicious TPLs from the host app based on the decompiled apk file by constructing the Component Invocation Graphs (CIG) and the call graphs of the suspicious libraries and then deleting the code related to the app; 
%(2) \textbf{Feature generation}, which generates the control flow graphs of each method in the libraries as the features to represent each suspicious library; 
%(3) \textbf{Library identification}, which identifies the library by comparing the features with the libraries in the database (if any) to see whether it exceeds the threshold, if there's no database exists or does not match any libraries in the database, it is considered as a new library and added to the library database. Therefore, the database can be extended automatically and iteratively.

%\xian{We implemented our TPL detection approach in a prototype tool named LibHunter. Figure~\ref{fig:libhunter_arch} illustrates the framework of our tool design. We mainly focus on two challenges in this work: code obfuscation and high-efficiency library identification. LibHunter also includes four key components: 1) preprocessing, 2) candidate libraries extraction, 3) feature generation, 4) Library identification.} 

%\sen{\bf What are the significant differences between other tools?}

%\subsection{Preprocessing}

%\xian{In this phase, we implement app decomplication. We employ a commonly-used reverse engineering tool Apktool~\cite{apktool} to decompile all Android apps in our depository.
%Apktool can help us disassemble AndroidManifest.xml file from the apk. We need to capture main components information from AndroidManifest.xml. Based on the information, we can distinguish the primary functional code and third-party code.}

\subsection{Module Decoupling}

\begin{figure}[!htb]
	\centering
	\includegraphics[width=1\linewidth]{example}\\
	\caption{Simplified package hierarchy and activity transitions (in green dashed line) of the app \texttt{de.emomedia}}
	\label{fig:pkghierarchy}	
\end{figure}

To extract library candidates inside the app under investigation, we first decompile the apk file by reverse engineering and extract the corresponding component data (e.g., package name, activities, services, and broadcast in AndroidManifest.xml file) related to the core logic of the app.
%To extract suspicious libraries inside the app under investigate, we first need to decompile the apk file by reverse engineering and extract the main component information (e.g., package name, Activities, and Services) related to the core logic of the app from the AndroidManifest.xml file. 
%Based on the components, we can split the core functionality code and the third-party library code.
In this paper, we define the package which includes the core logic code as the ``\textbf{\textit{primary}}'' module and third-party library parts as ``\textbf{\textit{non-primary}}'' module.
As shown in Figure~\ref{fig:pkghierarchy}, the app \texttt{de.emomedia}\footnote{\url{https://www.apkmonk.com/app/de.emomedia.plaetzchenfree/}} (called host app in this example) actually reuses some components of another package (i.e., \texttt{com.example}), and \texttt{com.example} intertwines with the logic of the main package, which usually happens when the host app reuses repackaged apps. 
Considering the above cases, we should consider these branches as primary.
However, existing techniques relying on package hierarchy or package names would definitely ignore the \texttt{com.example} package since parts of package name of the host app package structure (e.g., changing the branch ``com.example'' into any meaningless string or letter) can be obfuscated by some obfuscation tools.
%Besides, some obfuscation tools can also change parts of package name of the host app package structure, e.g., changing the branch ``com.example'' into any meaningless string or letter.
Therefore, these cases simply using the package name and package hierarchy structure to determine the boundary may not be accurate.
%In this case, both of them should be considered as the primary module. However, existing techniques relying on package hierarchy or package names would definitely ignore the \texttt{com.example} package and regard it as a TPL instead of the primary module. 
In this phase, our goal is to first identify the app package(s) of the host app (including \texttt{de.emomedia} and \texttt{com.example} in this case) by leveraging component transition graphs (CTG), and eliminate the primary module and identify different library candidates.

\vspace{1mm}
\noindent \textbf{Primary code elimination.}
To eliminate primary code, we propose to generate the component transition graph and leverage it to identify the primary modules.
Component transition graph is a multi-directed graph that can represent the invocation relations among basic components (i.e., \texttt{Activity}, \texttt{Service}, and \texttt{Broadcast Receiver}) in Android apps.  
\texttt{Activity} is a crucial component that users interact with and see directly when using apps. Each app usually has more than one activity, but with only one ``main'' activity (i.e., the first screen to appear when the use launches the app) such as login page and homepage of the app, which can be extracted all declared activity names from the \texttt{AndroidManifest.xml} file by specific tag name. 
A \texttt{Service} is a component which runs in the background to perform some long-running processing and associates with an app.
\texttt{Broadcast Receiver} is a component which can respond to broadcast messages from other applications or the Android system.
Actually, Android has four basic components, the other one is \texttt{Content Provider}, which offers the management service for the database and handles the user data. We exclude it since it has no transition relations with other components.

Actually, many existing work focuses on activity transition graph extraction{~\cite{chen2019storydroid,fan2018efficiently,yang2018static,octeau2015composite,azim2013targeted}}, however, they do not take the other two components into consideration. As we describe above, to ensure the performance of the module decoupling process, we need to identify all potential package(s) that belong to the host app. Therefore, we aim to generate a CTG, which includes different kinds of component types.
Basically, the transition relations between \texttt{Activity}, \texttt{Service} and \texttt{Broadcast Receiver} can be obtained through ``Intent,'' a messaging object which can start an activity, a service and a broadcast in the Android system. 
Actually, developers usually start activities by employing explicit calls to ensure the accurate transitions, while implicit calls are usually provided to other components for access.
Besides, we do not attempt to generate the complete CTG of the app to facilitate our decoupling process, instead, we need to generate the CTG that contains the main activity and the relations between different packages, which can guide us to remove the primary modules. Therefore, we also only consider explicit calls (i.e., start Activity using API ``startActivity()'', ``startActivityForResult()'', etc.), and ignore implicit calls between components whose call relations are determined at runtime.
Because the other packages that belong to host app do not use implicit calls to invoke the componets in the ``main'' package.
By leveraging the attribute of intent (i.e., which activity to start) and the transition method (e.g., ``startActivity()'' and ``startActivityForResult()''), we are able to construct the CTGs of one app.
For example, Activity \textit{A} can invoke the method ``startActivity(),'' ``startActivityForResult(),'' etc., in order to create Activity \textit{B}. We thus generate the transition: $A \rightarrow B$. In this way, we can obtain the nodes (components) and edges (transition relations) by parsing the intent, and confirm the real package(s) of the host app by using the partial relations.
%The generation phase is built on the static analysis framework, \textsc{Soot}.
%Some work implements the similar functionality on a famous static analysis framework, named \textsc{Soot}, however, the overhead is not the better choice compare with \textsc{A3E}. 
%Because, the completeness of component transition relations is not the main target for the further module decoupling.
%We only need to confirm the main CTG that contains the main activity extracted from manifest file.
%Therefore, we are able to confirm the real package(s) of the host app by using the partial relations.
%Note that we also only consider explicit calls, and ignore implicit calls between components whose call relations are determined at runtime.

For example, in Figure~\ref{fig:pkghierarchy}, we can generate the transition relations: \textit{MainActivity $\rightarrow$ AActivity, WeihnashActivity $\rightarrow$ BActivity}, thus the two packages are both regarded as primary modules.
Therefore, we identify the components that intertwines with the main logic (e.g., MainActivity, AActivity), and back track it to find the main directory (i.e., ``de'' and ``com.example'' in Figure~\ref{fig:pkghierarchy}). We thus delete all files in these directory.
In this way, we can delete all these primary
packages, but remain all the packages of third-party libraries.

%\subsubsection{Primary code elimination}
%Given the main CTG that contains the main activity, we backward traverse the main activity to obtain the root directory of the package, containing core functionalities of the app. 
%For example, in Figure~\ref{fig:pkghierarchy}, we identify the main activity is ``MainActivity'', and back track it to find the main directory (i.e., ``de''). We thus delete all files in this directory.
%We mentioned that some components in other packages may also be invoked by the main package, especially in the repackaged apps. 
%For example, \revise{``xxx'' in another package (i.e., \revise{xxx}) invokes ``xxx'', this package should also be considered as the main module since its components are invoked by the main package, and it intertwines with the logic of the main package (i.e., de.emomedia).} 
%Thus we also back track these files in other packages and consider them as the primary modules. 
%In this way, we can find all the packages which contain the primary code and delete all these primary
%packages, but remain all the packages of third-party libraries.

\vspace{1mm}
\noindent \textbf{TPL splitting.}
Apart from removing the primary code from the host app, we also require to split remaining files belonging to different libraries. Here,we use the package dependency graph (PDG) to conduct the module decoupling.

A PDG is defined as a 3-tuple $G = (N,E,W)$, where $N$ indicates a set of nodes in the graph, $E \subseteq (N \times N)$ is a set of edges, and $W$ is the weight value of each edge. Each node $n \in N$ represents a package (sub-package) or a class file. Each edge $e \in E$ indicates the relations between two nodes, and owns a weight $w$. In this paper, we consider 4 kinds of dependency relations and apply different weights for them since different dependency relations have different contribution to library splitting. Note that, we do not consider the intra package dependencies in this step.
\begin{itemize}
	\item \textit{Homogeneous relation (weight: 5)}, indicating parent-child relationship or siblings. If two nodes has the parent and child relationship or they share the same parent, we call they are homogeneous nodes.
	For example, in Figure~\ref{fig:pkghierarchy}, the node \texttt{helperactivities} and \texttt{plaerzchen} owns homogeneous relation, and \texttt{A Activity} and \texttt{B Activity} owns homogeneous relation.
	\item \textit{Class inheritance relation (weight: 4)}, indicating file level inheritance relations.
	\item \textit{Method call relation (weight: 2)}, indicating file-level relations via method calls.
	\item \textit{Field reference relation (weight: 1)}, indicating the file level relations via field reference.
	
\end{itemize}
The larger weight value is, the closer relation two nodes own.  Based on the relations together with the weight of each node,  
we employ the Hierarchical Agglomerative clustering algorithm~\cite{hierarchy_clustering} to split modules into different potential library candidates. {Specifically, we first compute the distance (measured by weight values) between every two files, and choose two files with the shortest distance to cluster them into one node for the next round. Such process is iterative until all the file are integrated into a tree. For each layer of the tree, we compute the distance between nodes, if the distance between two nodes exceeds a threshold (i.e.,0.15), we consider them as two separate packages (i.e., library). Finally, we obtain different library candidates.}

%Compared with previous module decoupling, our approach has several differences and improvement.


\subsection{Feature Generation}
After splitting the candidate libraries, we then extract features as a signature to represent each library. 
To defend against code obfuscation on libraries and detect new-emerging libraries, it is essential to generate relatively stable features to represent libraries. 
Existing work~\cite{LibD2017ICSE, LibRadar2016ICSE,libscout2016ccs,libpecker2018} extracts features such as opcode of CFG basic block, API calls and  fuzzy method signatures that are not resilient to common obfuscation techniques (e.g., dead code removal), and the number of opcode usually can reach to millions or billions level, which also costs a large amount of time for detection.
Thus in this paper, we extract CFGs as the feature since: (1) CFG is relatively stable, resilient to both the code level and the package name/structure level obfuscation, and is difficult to be modified by utilizing existing obfuscation techniques~\cite{roy2007survey}. Existing obfuscators just implement simple control-flow obfuscation, like inserting opaque predicates, but it is difficult to be statically determined~\cite{CFO2016}; (2) CFG keeps the semantic information and ensures the accuracy to some extent~\cite{chen14ICSE}. 
The feature generation consists of two primary steps: 1) generate the control-flow graphs (CFGs) for candidate libraries 2) change the CFGs into the birthmarks (i.e., signatures) to represent the third-party libraries.
%\sen{Also need to introduce why we extract CFG on the dex level.}


Specifically, we first generate CFG from Dex file for each method in the candidate libraries, and use breadth-first traversal to assign each node a serial number which is then used to represent the control flows between nodes. 
%\revise{We highlight that using Dex file to extract CFG }
We then convert the CFGs into signatures based on the assigned serial numbers of each node to represent each third-party library, in the form of \texttt{[node count, edge adjacency list]}, 
where the package structure is
the adjacency list is represented as: \texttt{[$parent_1$ -> ($child_1$,$child_2$,...), $parent_2$ -> ...]}. 
Besides, for each method, we also extract the method location in the package structure which can be used to confirm the identified libraries, or used as the library name if it is not obfuscated and is a newly-emerging library. 
Finally, each library is represented as several CFG signatures.
%We use the set of edge adjacency list of CFG to indicate the library candidate. 
%For each method in the library, we generate the signature 
%For example, a signature of CFG is as follows:

%\begin{lstlisting}[caption=signature example]
%com/example/class.a()V;4;0:1,2;1:3;2:3,0
%\end{lstlisting}

%The package structure is ``com/example/class.a()V'', there are four nodes in this CFG. We can break out the adjacency list:
%\begin{lstlisting}
%0:1,2
%1:3
%2:3,0
%\end{lstlisting}

%Which means the Node 0 points to Node 1 and Node 2. Node1 points to Node 3 and Node 2 branches to Node 3 and Node 0. We use the Breadth-First-Search (BFS) algorithm to get the node number.

%We generate the Control Flow Graph (CFG) for each method from each class files of the remaining candidate packages, and use \revise{this algorithm~\cite{chen14ICSE} (describe more about it.)} to generate a signature for each CFG.


\subsection{Library Identification}
%\sen{why use threshold?}
For a given Android app, after generating signatures for each candidate library, we compare the signatures with the existing ones in the database (if any), and identify the specific libraries. Our proposed library identification approach can also identify libraries that do not exist in the constructed library database. We describe the details as follows. 

Actually, LibHunter does not require a library database for comparison. From the beginning, if there is not such a lib database for comparison, it directly creates one, and stores the currently identified one together with its CFG signatures to the database. The initially created database can later be used for comparison with the candidate ones and can also be extended by adding newly identified libraries.

\noindent \textbf{Lib identification.}
If there exists a library database for comparison, LibHunter compares the CFG signatures of the candidate library with the ones in the database. For each signature-comparing pair, we only regard them as the same one if their signatures are exactly the same. 
{Note that each library is represented as several signatures, thus we consider two libraries as the same one only if the percentage of the same signatures exceeds a threshold (i.e., similarity threshold).} 
Here, we use a similarity threshold between the candidate library and the reference libraries in the database instead of employing the extract matching mechanism since we should consider the code obfuscation and lib spliting sometime cannot achieve 100\% accuracy.
The similarity of two libraries is computed using Jaccard similarity as follows:
\[
J(Lib_a, Lib_b) = \frac{\left |S_{Lib_a}\bigcap S_{Lib_b}\right |}{\left |S_{Lib_a}\bigcup  S_{Lib_b}\right |}
\]
where $S_{Lib_a}$ and $S_{Lib_b}$ represent the signatures of libraries $a$ and $b$, respectively. $J(Lib_a, Lib_b) \in [0, 1]$.
If the similarity of two libraries exceeds a threshold $\alpha$, we consider them as the same one, otherwise, they are considered as different ones. After comparison with all the libraries in the existing database, if there is no such a library whose similarity with the candidate library exceeds the threshold, we consider it as a newly identified one, and add the signatures of it to the existing database with the library name.
However, libraries may be obfuscated without real library names, in this case, we only add the signatures into the database without the library name. 
When there is another library (without obfuscation) coming with high similarity (i.e., exceeds the threshold $\alpha$) to the obfuscated one, we assign the library name to the obfuscated library in the database.



\noindent \textbf{Enable fast comparison.}
%\sen{concrete implementation?}
Comparing CFG signatures of each method is a time-consuming task. To achieve fast comparison, we store the signatures of each library in a descending order. Given the signatures of the candidate library, we compare it with the signatures of the libraries in the database by utilizing binary search, which significantly accelerates the speed of comparison.

%\sen{what's this?}
%\revise{Our method can tolerate the libraries modification, both the code and the package name/structure. (not sure. need more discussion.)}
%Even though Hu et al.~\cite{Duet2014Wisec} pointed out that more than 80\% of third-party libraries are used without
%modification by developers in their dataset of 100,000 Google Play apps, a recent study~\cite{LibD2017ICSE} also shows that the same library may be mutated due to different visions. Our method can handle this problem well.


%\sen{\bf I am not sure whether we need to mention some security to the identified libs?}


==> Tool.tex <==
\begin{table*}[thpb]
	
	\centering
	%\small
	\caption{Overview of the existing available TPL detection tools.}
	\scalebox{0.90}{
		\begin{tabular}{lc|c|ccc|c}
			\hline
			\multirow{2}{*}{\textbf{Tool}}  &  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} \textbf{Preprocessing}\\ \textbf{Tool}\end{tabular}} &
			\multirow{2}{*}{\textbf{Module decoupling}} & \multicolumn{3}{c|}{\textbf{Feature Extraction}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} \textbf{Library}\\ \textbf{Identification}\end{tabular}} \\
			\cline{4-6}
			& &   & \multicolumn{1}{c}{\textbf{Feature}} & \textbf{Granularity} & \multicolumn{1}{c|}{\textbf{Method}} & \\
			
			\hline \hline
			\rowcolor{gray!20}
			\textbf{\textit{LibPecker}}  & \begin{tabular}[c]{@{}c@{}} Apktool,\\ Androguard\end{tabular} & PN, PHS   & Class Dependency & Class & Hash & Fuzzy Class Matching\\
			
			\textbf{\textit{ORLIS}}     &  Soot & -  & Fuzzy Method Signature & Class & Hash & Similarity Comparison\\
			
			\rowcolor{gray!20}			
			\textbf{\textit{LibRadar}}    & Apktool & PN, PHS   & API calls & package & Hash & Clustering\\
			
			\textbf{\textit{LibScout}}  & - & - & Fuzzy Method Signature & Package & Merkle Tree & Similarity Comparison\\
			
			\rowcolor{gray!20}
			\textbf{\textit{LibD$^*$}}  &\begin{tabular}[c]{@{}c@{}} Apktool,\\ Androguard\end{tabular}  & PN, HG  & Opcode& Package & Hash & Clustering\\
			\hline
		\end{tabular}
	}
	\label{tbl:TPL_tech_CMP}
	
	\begin{flushleft}
		\begin{center}
			\textit{GT: ground truth, PN: package name, PHS: package hierarchy structure, HG: homogeny graph, %PDG: package dependency graph. 
				\\
				\textbf{LibD$^*$}: publicly available, but was reported an error by the owner~\cite{libd_error}, thus we excluded it for comparison.
			}
		\end{center}
	\end{flushleft}
\end{table*}

\section{Implementation}
\label{sec:tool}

We release \mytool as an online web service,\footnote{https://example.com} which takes as input an Android app, and identifies the libraries used by the app.
\mytool is implemented in 2,000+ lines of python code.
We employ a commonly-used reverse engineering tool \textsc{Apktool}~\cite{apktool} to decompile the Android apps. To obtain the primary modules that need to be eliminate, we build on \textsc{Gator} to construct the CTG between different types of components. 
We then employ \revise{XX} and \revise{XX} to obtain the call relations and other package dependencies, in order to split out different libraries.
To identify the names of the split candidate libraries, we set the similarity threshold $\alpha = 80\%$ between the candidate library and the reference libraries in our experiment.
We maintain a library database containing all identified libraries together with their signatures, and automatically extend it by adding newly identified ones.
Currently our database contains 2,115 libraries for comparison.


